Merging Hierarchical Triple Black Hole Systems with Intermediate-mass Black Holes in Population III Star Clusters

Theoretical predictions suggest that very massive stars have the potential to form through multiple collisions and eventually evolve into intermediate-mass black holes (IMBHs) within Population III star clusters embedded in mini dark matter haloes. In this study, we investigate the long-term evolution of Population III star clusters, including models with a primordial binary fraction of $f_{\rm b}=0$ and 1, using the $N$-body simulation code PETAR. We comprehensively examine the phenomenon of hierarchical triple black holes in the clusters, specifically focusing on their merging inner binary black holes (BBHs), with post-Newtonian correction, by using the TSUNAMI code. Our findings suggest a high likelihood of the inner BBHs containing IMBHs with masses on the order of $\mathcal{O}(100)M_{\odot}$, and as a result, their merger rate could be up to $0.1{\rm Gpc}^{-3}{\rm yr}^{-3}$. The orbital eccentricities of some merging inner BBHs oscillate over time periodically, known as the Kozai-Lidov oscillation, due to dynamical perturbations. Detectable merging inner BBHs for mHz GW detectors LISA/TianQin/Taiji concentrate within $z<3$. More distant sources would be detectable for CE/ET/LIGO/KAGRA/DECIGO, which are sensitive from $\mathcal{O}(0.1)$Hz to $\mathcal{O}(100)$Hz. Furthermore, compared with merging isolated BBHs, merging inner BBHs affected by dynamical perturbations from tertiary BHs tend to have higher eccentricities, with a significant fraction of sources with eccentricities closing to 1 at mHz bands. GW observations would help constrain formation channels of merging BBHs, whether through isolated evolution or dynamical interaction, by examining eccentricities.

==> makefile <==
tex=latexmk
#pdf_browser=/mnt/c/Program\ Files\ \(x86\)/Foxit\ Software/Foxit\ Reader/Foxit\ PDF\ Reader/FoxitPDFReader.exe#evince
pdf_browser=open
target1=main.tex
target2=main.pdf
main:
	$(tex) -pdf -bibtex $(target1)  # -pdf -bibtex分别是将.tex编译为pdf文件和处理参考文献
	$(pdf_browser) $(target2)       # 浏览pdf文件

clean:
	$(tex) -CA # 删除编译后产生的无用文件
	-rm *.bbl  # 删除后缀为.bbl的所有文件 
	-rm *.xml  # 删除.xml文件

